The Mariana Environmental Disaster and its Labor Market Effects

This paper examines the labor market impacts of the 2015 Mariana Dam disaster in Brazil. It contrasts two theoretical models: an urban spatial equilibrium model and a factor of production model, with diverging perspectives on environmental influences on labor outcomes. Utilizing rich national administrative and spatial data, the study reveals that the unusual environmental alteration, with minimal human capital loss, primarily affected outcomes via the factor of production channel. Nevertheless, spatial equilibrium dynamics are discernible within certain market segments. This research contributes to the growing literature on environmental changes and its economic consequences.

==> tab_es_010203_dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.008} & \num{0.075}*** & \num{0.010} & \num{0.006} & \num{0.072}** & \num{0.009}\\
 & (\num{0.024}) & (\num{0.025}) & (\num{0.028}) & (\num{0.024}) & (\num{0.027}) & (\num{0.028})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.385} & \num{0.031} & \num{0.424} & \num{0.392} & \num{0.032} & \num{0.429}\\
R2 Adj. & \num{0.180} & \num{0.031} & \num{-0.263} & \num{0.190} & \num{0.032} & \num{-0.252}\\
RMSE & \num{0.384} & \num{0.482} & \num{0.372} & \num{0.386} & \num{0.482} & \num{0.373}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_010203_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.035}*** & \num{-0.066}** & \num{-0.027}** & \num{-0.033}*** & \num{-0.084}*** & \num{-0.024}*\\
 & (\num{0.008}) & (\num{0.024}) & (\num{0.010}) & (\num{0.010}) & (\num{0.028}) & (\num{0.012})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.834} & \num{0.343} & \num{0.856} & \num{0.839} & \num{0.356} & \num{0.860}\\
R2 Adj. & \num{0.778} & \num{0.343} & \num{0.685} & \num{0.785} & \num{0.356} & \num{0.692}\\
RMSE & \num{0.262} & \num{0.521} & \num{0.243} & \num{0.264} & \num{0.522} & \num{0.244}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_010203_mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.004} & \num{0.021}** & \num{0.009} & \num{-0.005} & \num{0.018} & \num{0.009}\\
 & (\num{0.020}) & (\num{0.010}) & (\num{0.026}) & (\num{0.020}) & (\num{0.011}) & (\num{0.026})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.513} & \num{0.042} & \num{0.585} & \num{0.518} & \num{0.039} & \num{0.586}\\
R2 Adj. & \num{0.343} & \num{0.042} & \num{0.055} & \num{0.350} & \num{0.039} & \num{0.056}\\
RMSE & \num{0.293} & \num{0.411} & \num{0.271} & \num{0.296} & \num{0.412} & \num{0.272}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_03_dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.006} & \num{-0.085}*** & \num{0.021} & \num{-0.105} & \num{-0.103}*** & \num{-0.074}\\
 & (\num{0.029}) & (\num{0.016}) & (\num{0.033}) & (\num{0.063}) & (\num{0.032}) & (\num{0.083})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.385} & \num{0.031} & \num{0.424} & \num{0.392} & \num{0.032} & \num{0.429}\\
R2 Adj. & \num{0.180} & \num{0.031} & \num{-0.263} & \num{0.190} & \num{0.032} & \num{-0.252}\\
RMSE & \num{0.384} & \num{0.482} & \num{0.372} & \num{0.386} & \num{0.482} & \num{0.373}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_03_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
    Treat x Post & \num{-0.066}*** & \num{0.026} & \num{-0.070}*** & \num{-0.113}*** & \num{-0.022} & \num{-0.125}***\\
 & (\num{0.010}) & (\num{0.025}) & (\num{0.009}) & (\num{0.019}) & (\num{0.031}) & (\num{0.016})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.834} & \num{0.343} & \num{0.856} & \num{0.839} & \num{0.356} & \num{0.860}\\
R2 Adj. & \num{0.778} & \num{0.343} & \num{0.685} & \num{0.785} & \num{0.356} & \num{0.692}\\
RMSE & \num{0.262} & \num{0.521} & \num{0.243} & \num{0.264} & \num{0.522} & \num{0.244}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_03_mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.076}** & \num{-0.001} & \num{0.094}*** & \num{0.049} & \num{-0.014} & \num{0.101}**\\
 & (\num{0.034}) & (\num{0.015}) & (\num{0.017}) & (\num{0.057}) & (\num{0.021}) & (\num{0.036})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.513} & \num{0.042} & \num{0.585} & \num{0.518} & \num{0.039} & \num{0.586}\\
R2 Adj. & \num{0.343} & \num{0.042} & \num{0.055} & \num{0.350} & \num{0.039} & \num{0.056}\\
RMSE & \num{0.293} & \num{0.411} & \num{0.271} & \num{0.296} & \num{0.412} & \num{0.272}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es__dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.021} & \num{-0.002} & \num{-0.023} & \num{-0.035} & \num{-0.001} & \num{-0.024}\\
 & (\num{0.031}) & (\num{0.008}) & (\num{0.015}) & (\num{0.026}) & (\num{0.009}) & (\num{0.016})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.385} & \num{0.031} & \num{0.424} & \num{0.393} & \num{0.032} & \num{0.429}\\
R2 Adj. & \num{0.180} & \num{0.031} & \num{-0.263} & \num{0.190} & \num{0.032} & \num{-0.252}\\
RMSE & \num{0.384} & \num{0.482} & \num{0.372} & \num{0.386} & \num{0.482} & \num{0.373}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es__log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.013} & \num{-0.009} & \num{0.003} & \num{0.015} & \num{-0.019} & \num{0.003}\\
 & (\num{0.009}) & (\num{0.013}) & (\num{0.012}) & (\num{0.013}) & (\num{0.015}) & (\num{0.017})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.834} & \num{0.343} & \num{0.856} & \num{0.839} & \num{0.356} & \num{0.860}\\
R2 Adj. & \num{0.778} & \num{0.343} & \num{0.685} & \num{0.785} & \num{0.356} & \num{0.692}\\
RMSE & \num{0.262} & \num{0.521} & \num{0.243} & \num{0.264} & \num{0.522} & \num{0.244}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es__mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.018} & \num{0.010} & \num{-0.016} & \num{-0.035} & \num{0.006} & \num{-0.017}\\
 & (\num{0.040}) & (\num{0.006}) & (\num{0.010}) & (\num{0.035}) & (\num{0.007}) & (\num{0.012})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.513} & \num{0.042} & \num{0.585} & \num{0.518} & \num{0.039} & \num{0.586}\\
R2 Adj. & \num{0.343} & \num{0.042} & \num{0.055} & \num{0.351} & \num{0.039} & \num{0.056}\\
RMSE & \num{0.293} & \num{0.411} & \num{0.271} & \num{0.296} & \num{0.412} & \num{0.272}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_office_dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.012} & \num{-0.053}*** & \num{-0.017}* & \num{-0.021} & \num{-0.053}*** & \num{-0.018}\\
 & (\num{0.016}) & (\num{0.007}) & (\num{0.009}) & (\num{0.023}) & (\num{0.009}) & (\num{0.012})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.385} & \num{0.031} & \num{0.424} & \num{0.392} & \num{0.032} & \num{0.429}\\
R2 Adj. & \num{0.180} & \num{0.031} & \num{-0.263} & \num{0.190} & \num{0.032} & \num{-0.252}\\
RMSE & \num{0.384} & \num{0.482} & \num{0.372} & \num{0.386} & \num{0.482} & \num{0.373}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_office_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.023}* & \num{-0.046}* & \num{0.022}* & \num{0.025}* & \num{-0.076}** & \num{0.022}\\
 & (\num{0.012}) & (\num{0.024}) & (\num{0.012}) & (\num{0.013}) & (\num{0.029}) & (\num{0.014})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.834} & \num{0.343} & \num{0.856} & \num{0.839} & \num{0.356} & \num{0.860}\\
R2 Adj. & \num{0.778} & \num{0.343} & \num{0.685} & \num{0.785} & \num{0.356} & \num{0.692}\\
RMSE & \num{0.262} & \num{0.521} & \num{0.243} & \num{0.264} & \num{0.522} & \num{0.244}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644} & \num{5100644}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_es_office_mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.007} & \num{-0.022}*** & \num{0.002} & \num{-0.004} & \num{-0.026}*** & \num{0.000}\\
 & (\num{0.017}) & (\num{0.007}) & (\num{0.006}) & (\num{0.026}) & (\num{0.005}) & (\num{0.007})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.513} & \num{0.042} & \num{0.585} & \num{0.518} & \num{0.039} & \num{0.586}\\
R2 Adj. & \num{0.343} & \num{0.042} & \num{0.055} & \num{0.350} & \num{0.039} & \num{0.056}\\
RMSE & \num{0.293} & \num{0.411} & \num{0.271} & \num{0.296} & \num{0.412} & \num{0.272}\\
N Clusters & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000} & \num{16.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754} & \num{4351754}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_ironbelt_010203_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.063}** & \num{-0.271}*** & \num{-0.055}*** & \num{-0.025} & \num{-0.265}*** & \num{-0.025}\\
 & (\num{0.023}) & (\num{0.032}) & (\num{0.011}) & (\num{0.023}) & (\num{0.019}) & (\num{0.020})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.894} & \num{0.397} & \num{0.911} & \num{0.885} & \num{0.401} & \num{0.897}\\
R2 Adj. & \num{0.846} & \num{0.397} & \num{0.730} & \num{0.832} & \num{0.401} & \num{0.689}\\
RMSE & \num{0.233} & \num{0.556} & \num{0.214} & \num{0.238} & \num{0.556} & \num{0.215}\\
N Clusters & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_ironbelt_07_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Iron Mining: Treat x Post & \num{-0.196}*** & \num{0.368}*** & \num{-0.297}*** & \num{-0.240}*** & \num{0.510}*** & \num{-0.294}***\\
 & (\num{0.017}) & (\num{0.023}) & (\num{0.009}) & (\num{0.028}) & (\num{0.035}) & (\num{0.005})\\
\midrule
Rural Activities: Treat x Post & \num{-0.063}** & \num{-0.271}*** & \num{-0.055}*** & \num{-0.025} & \num{-0.265}*** & \num{-0.025}\\
 & (\num{0.023}) & (\num{0.032}) & (\num{0.011}) & (\num{0.023}) & (\num{0.019}) & (\num{0.020})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
N Clusters & \num{12} & \num{12} & \num{12} & \num{12} & \num{12} & \num{12}\\
N & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721}\\
        \bottomrule
\end{tabular}
        \end{adjustbox}
        \begin{flushleft}
            \parbox{\textwidth}{\footnotesize
            \textsuperscript{1} Standard-errors are clustered by municipality.\\
            \textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01\\
            \textsuperscript{3} Covariates used for the municipality fixed-effect model are age, age-squared, education level, race, and gender.\\
            \textsuperscript{4} Covariates used for propensity score estimation in DR models are age, tenure, education level, gender, race, worker's occupation, and the firm's main economic activity.\\
            \textsuperscript{5} Iron Mining activity code is 07. Rural Activities correspond to agriculture (01), forestry (02), and fishing (03).\\
        \end{flushleft}



==> tab_ironbelt__dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.003} & \num{-0.001} & \num{-0.005} & \num{0.041} & \num{-0.001} & \num{0.010}\\
 & (\num{0.036}) & (\num{0.019}) & (\num{0.021}) & (\num{0.026}) & (\num{0.020}) & (\num{0.021})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.435} & \num{0.043} & \num{0.472} & \num{0.430} & \num{0.036} & \num{0.457}\\
R2 Adj. & \num{0.176} & \num{0.043} & \num{-0.595} & \num{0.168} & \num{0.036} & \num{-0.641}\\
RMSE & \num{0.365} & \num{0.476} & \num{0.353} & \num{0.368} & \num{0.476} & \num{0.354}\\
N Clusters & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_ironbelt__log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.066}*** & \num{-0.035}** & \num{-0.052}*** & \num{-0.054}*** & \num{-0.029}** & \num{-0.055}***\\
 & (\num{0.016}) & (\num{0.011}) & (\num{0.010}) & (\num{0.013}) & (\num{0.012}) & (\num{0.009})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.894} & \num{0.397} & \num{0.911} & \num{0.885} & \num{0.401} & \num{0.897}\\
R2 Adj. & \num{0.846} & \num{0.397} & \num{0.730} & \num{0.832} & \num{0.401} & \num{0.689}\\
RMSE & \num{0.233} & \num{0.556} & \num{0.214} & \num{0.238} & \num{0.556} & \num{0.215}\\
N Clusters & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_ironbelt__mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.034} & \num{0.004} & \num{-0.036} & \num{0.013} & \num{0.008} & \num{-0.024}\\
 & (\num{0.047}) & (\num{0.016}) & (\num{0.024}) & (\num{0.029}) & (\num{0.016}) & (\num{0.023})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.590} & \num{0.085} & \num{0.638} & \num{0.599} & \num{0.081} & \num{0.636}\\
R2 Adj. & \num{0.390} & \num{0.085} & \num{-0.173} & \num{0.405} & \num{0.081} & \num{-0.179}\\
RMSE & \num{0.289} & \num{0.432} & \num{0.271} & \num{0.293} & \num{0.432} & \num{0.272}\\
N Clusters & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{1348847} & \num{1348847} & \num{1348847} & \num{1348847} & \num{1348847} & \num{1348847}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_ironbelt_office_dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.042} & \num{-0.027} & \num{-0.048}** & \num{-0.037}** & \num{-0.033}*** & \num{-0.054}***\\
 & (\num{0.029}) & (\num{0.016}) & (\num{0.018}) & (\num{0.014}) & (\num{0.010}) & (\num{0.010})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.435} & \num{0.043} & \num{0.472} & \num{0.430} & \num{0.036} & \num{0.457}\\
R2 Adj. & \num{0.176} & \num{0.043} & \num{-0.595} & \num{0.168} & \num{0.036} & \num{-0.641}\\
RMSE & \num{0.365} & \num{0.476} & \num{0.353} & \num{0.368} & \num{0.476} & \num{0.354}\\
N Clusters & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_ironbelt_office_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.014} & \num{-0.036} & \num{0.020} & \num{0.052}** & \num{-0.046}** & \num{0.051}**\\
 & (\num{0.018}) & (\num{0.022}) & (\num{0.011}) & (\num{0.023}) & (\num{0.017}) & (\num{0.023})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.894} & \num{0.397} & \num{0.911} & \num{0.885} & \num{0.401} & \num{0.897}\\
R2 Adj. & \num{0.846} & \num{0.397} & \num{0.730} & \num{0.832} & \num{0.401} & \num{0.689}\\
RMSE & \num{0.233} & \num{0.556} & \num{0.214} & \num{0.238} & \num{0.556} & \num{0.215}\\
N Clusters & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721} & \num{1567721}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_ironbelt_office_mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.059} & \num{-0.012} & \num{-0.062}** & \num{-0.033}** & \num{-0.002} & \num{-0.052}***\\
 & (\num{0.042}) & (\num{0.016}) & (\num{0.021}) & (\num{0.013}) & (\num{0.009}) & (\num{0.014})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.590} & \num{0.085} & \num{0.638} & \num{0.599} & \num{0.081} & \num{0.636}\\
R2 Adj. & \num{0.390} & \num{0.085} & \num{-0.173} & \num{0.405} & \num{0.081} & \num{-0.179}\\
RMSE & \num{0.289} & \num{0.432} & \num{0.271} & \num{0.293} & \num{0.432} & \num{0.272}\\
N Clusters & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000} & \num{12.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{1348847} & \num{1348847} & \num{1348847} & \num{1348847} & \num{1348847} & \num{1348847}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas_010203_dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.011} & \num{-0.023} & \num{0.027} & \num{-0.079}** & \num{-0.117} & \num{-0.004}\\
 & (\num{0.029}) & (\num{0.060}) & (\num{0.023}) & (\num{0.040}) & (\num{0.072}) & (\num{0.054})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.388} & \num{0.049} & \num{0.427} & \num{0.394} & \num{0.048} & \num{0.434}\\
R2 Adj. & \num{0.221} & \num{0.049} & \num{-0.096} & \num{0.229} & \num{0.048} & \num{-0.083}\\
RMSE & \num{0.383} & \num{0.477} & \num{0.370} & \num{0.383} & \num{0.477} & \num{0.371}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas_010203_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.061}*** & \num{-0.124}*** & \num{-0.045}*** & \num{-0.047}* & \num{-0.140}*** & \num{-0.038}\\
 & (\num{0.012}) & (\num{0.017}) & (\num{0.010}) & (\num{0.027}) & (\num{0.030}) & (\num{0.029})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.823} & \num{0.361} & \num{0.849} & \num{0.858} & \num{0.379} & \num{0.878}\\
R2 Adj. & \num{0.775} & \num{0.361} & \num{0.711} & \num{0.819} & \num{0.379} & \num{0.766}\\
RMSE & \num{0.259} & \num{0.492} & \num{0.239} & \num{0.260} & \num{0.497} & \num{0.240}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas_010203_mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.026} & \num{-0.053} & \num{0.009} & \num{-0.055}* & \num{-0.085} & \num{0.010}\\
 & (\num{0.019}) & (\num{0.032}) & (\num{0.014}) & (\num{0.028}) & (\num{0.055}) & (\num{0.031})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.507} & \num{0.054} & \num{0.613} & \num{0.523} & \num{0.056} & \num{0.617}\\
R2 Adj. & \num{0.366} & \num{0.054} & \num{0.239} & \num{0.387} & \num{0.056} & \num{0.246}\\
RMSE & \num{0.262} & \num{0.362} & \num{0.232} & \num{0.263} & \num{0.363} & \num{0.232}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas__dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.019}** & \num{-0.006} & \num{0.023}** & \num{0.019}** & \num{-0.014} & \num{0.020}\\
 & (\num{0.008}) & (\num{0.008}) & (\num{0.009}) & (\num{0.009}) & (\num{0.010}) & (\num{0.012})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.388} & \num{0.049} & \num{0.427} & \num{0.394} & \num{0.048} & \num{0.434}\\
R2 Adj. & \num{0.221} & \num{0.049} & \num{-0.096} & \num{0.229} & \num{0.048} & \num{-0.082}\\
RMSE & \num{0.383} & \num{0.477} & \num{0.370} & \num{0.383} & \num{0.477} & \num{0.371}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas__log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{-0.038}*** & \num{-0.049}** & \num{-0.035}** & \num{-0.058}*** & \num{-0.083}** & \num{-0.056}**\\
 & (\num{0.014}) & (\num{0.023}) & (\num{0.015}) & (\num{0.021}) & (\num{0.034}) & (\num{0.023})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.824} & \num{0.362} & \num{0.849} & \num{0.858} & \num{0.379} & \num{0.878}\\
R2 Adj. & \num{0.775} & \num{0.362} & \num{0.711} & \num{0.819} & \num{0.379} & \num{0.767}\\
RMSE & \num{0.259} & \num{0.492} & \num{0.239} & \num{0.260} & \num{0.497} & \num{0.240}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas__mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.011}* & \num{-0.017}* & \num{0.010} & \num{0.015}*** & \num{-0.021}* & \num{0.008}\\
 & (\num{0.006}) & (\num{0.009}) & (\num{0.007}) & (\num{0.005}) & (\num{0.011}) & (\num{0.006})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.507} & \num{0.054} & \num{0.613} & \num{0.523} & \num{0.056} & \num{0.617}\\
R2 Adj. & \num{0.366} & \num{0.054} & \num{0.239} & \num{0.387} & \num{0.056} & \num{0.246}\\
RMSE & \num{0.262} & \num{0.362} & \num{0.232} & \num{0.263} & \num{0.363} & \num{0.232}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas_office_dismissed.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.012}*** & \num{-0.040}*** & \num{0.012} & \num{0.012}*** & \num{-0.026}** & \num{0.011}\\
 & (\num{0.003}) & (\num{0.005}) & (\num{0.008}) & (\num{0.003}) & (\num{0.011}) & (\num{0.008})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.388} & \num{0.049} & \num{0.427} & \num{0.394} & \num{0.048} & \num{0.434}\\
R2 Adj. & \num{0.221} & \num{0.049} & \num{-0.096} & \num{0.229} & \num{0.048} & \num{-0.083}\\
RMSE & \num{0.383} & \num{0.477} & \num{0.370} & \num{0.383} & \num{0.477} & \num{0.371}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas_office_log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.001} & \num{-0.012} & \num{0.004} & \num{0.008} & \num{-0.066} & \num{0.013}\\
 & (\num{0.011}) & (\num{0.039}) & (\num{0.010}) & (\num{0.010}) & (\num{0.051}) & (\num{0.009})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.823} & \num{0.361} & \num{0.849} & \num{0.858} & \num{0.379} & \num{0.878}\\
R2 Adj. & \num{0.775} & \num{0.361} & \num{0.711} & \num{0.819} & \num{0.379} & \num{0.766}\\
RMSE & \num{0.259} & \num{0.492} & \num{0.239} & \num{0.260} & \num{0.497} & \num{0.240}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590} & \num{19334590}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_minas_office_mover.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.014}*** & \num{-0.022}** & \num{0.012}** & \num{0.012}*** & \num{-0.015}*** & \num{0.011}**\\
 & (\num{0.004}) & (\num{0.010}) & (\num{0.006}) & (\num{0.003}) & (\num{0.005}) & (\num{0.005})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.507} & \num{0.054} & \num{0.613} & \num{0.523} & \num{0.056} & \num{0.617}\\
R2 Adj. & \num{0.366} & \num{0.054} & \num{0.239} & \num{0.387} & \num{0.056} & \num{0.246}\\
RMSE & \num{0.262} & \num{0.362} & \num{0.232} & \num{0.263} & \num{0.363} & \num{0.232}\\
N Clusters & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000} & \num{323.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725} & \num{16541725}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_placebo_minas__log_wage.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat x Post & \num{0.009} & \num{0.005} & \num{0.009} & \num{0.009} & \num{0.005} & \num{0.009}\\
 & (\num{0.007}) & (\num{0.006}) & (\num{0.007}) & (\num{0.007}) & (\num{0.006}) & (\num{0.007})\\
\midrule
Individual FE & X &  & X & X &  & X\\
Individual x Municipality FE &  &  & X &  &  & X\\
Municipality FE &  & X & X &  & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.818} & \num{0.366} & \num{0.844} & \num{0.818} & \num{0.368} & \num{0.845}\\
R2 Adj. & \num{0.769} & \num{0.366} & \num{0.704} & \num{0.769} & \num{0.367} & \num{0.705}\\
RMSE & \num{0.261} & \num{0.488} & \num{0.242} & \num{0.261} & \num{0.488} & \num{0.242}\\
N Clusters & \num{279.000} & \num{279.000} & \num{279.000} & \num{279.000} & \num{279.000} & \num{279.000}\\
NA & NA & NA & NA & NA & NA & \vphantom{1} NA\\
NA & NA & NA & NA & NA & NA & NA\\
N & \num{16417923} & \num{16417923} & \num{16417923} & \num{16417923} & \num{16417923} & \num{16417923}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}

